Servos for Local Map Exploration Onboard Nonholonomic Vehicles for Extremum Seeking

Extremum seeking control (ESC) often employs perturbation-based estimates of derivatives for some sensor field or cost function. These estimates are generally obtained by simply multiplying the output of a single-unit sensor by some time-varying function. Previous work has focused on sinusoidal perturbations to generate derivative estimates with results for arbitrary order derivatives of scalar maps or higher up to third-order derivatives of multivariable maps. This work extends the perturbations from sinusoidal to bounded periodic or almost periodic functions and considers multivariable maps. A necessary and sufficient condition is given for determining if time-varying functions exist for estimating arbitrary order derivatives of multivariable maps for any given bounded periodic or almost periodic dither signal. These results are then used in a source seeking controller for a nonholonomic vehicle with a sensor actuated by servo. The conducted simulation and real-world experiments demonstrate that by distributing the local map exploration to a servo, the nonholonomic vehicle was able to achieve a faster convergence to the source.

==> figures/tik-images/acoustic-source.tex <==
\begin{tikzpicture}%
  % Place the PNG image as a node
  \node[anchor=south west, inner sep=0] (image) at (0,0) {%
    \includegraphics[width=0.7\textwidth]{figures/robot/acoustic-source.jpg}%
  };
  
  \begin{scope}[
    x={(image.south east)},%
    y={(image.north west)}
  ]
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % 1) Sound source
    \node[
      draw=red,
      thick,
      rectangle,
      fill = white!80,
      text=red,
      font=\bfseries\Huge,  % Make text bold & larger
      inner sep=5pt          % Extra padding inside the box
    ]
    at (0.35, 0.85) (source) {Sound Source};
    \draw[red, above,ultra thick] (0.4, 0.5) circle (0.05);
    \draw[->,red, ultra thick] (source.south) -- (0.4,0.56);
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % 2) Vicon LED Detectors draw
    \node[
      draw=red,
      thick,
      rectangle,
      fill = white!80,
      text=red,
      font=\bfseries\Huge,  % Make text bold & larger
      inner sep=5pt          % Extra padding inside the box
    ]
    at (0.33, 0.25) (vicon) {Vicon LED Detectors};
    \draw[red, right,ultra thick] (0.68,0.45) circle (0.05); 
    \draw[->,red,ultra thick] (vicon.north) -- (0.65,0.4);
    
  \end{scope}
\end{tikzpicture}

==> figures/tik-images/lab-test-area.tex <==
\begin{tikzpicture}%
  % Place the PNG image as a node
  \node[anchor=south west, inner sep=0] (image) at (0,0) {%
    \includegraphics[width=0.6\textwidth]{figures/robot/rot-sensor-lab-test-area.jpg}%
  };
  \begin{scope}[
    x={(image.south east)},%
    y={(image.north west)}
  ]
    %
    % 1) Draw the x-y at coordinates for the robots
    \draw[->,red, ultra thick] (0.75, 0.7) -- (0.5,0.7);
    \draw[->,red, ultra thick] (0.75, 0.7) -- (0.75,0.5);
    \node[red,right,font=\bfseries\large] at (.77,.6) {Y};
    \node[red,right,font=\bfseries\large] at (.6,.73) {X};

    % 2) Seeker node
    \node[
      draw=red,
      thick,
      rectangle,
      fill = white!80,
      text=red,
      font=\bfseries\LARGE,  % Make text bold & larger
      inner sep=5pt          % Extra padding inside the box
    ]
    at (0.65, 0.88) {Seeker};
    \node[
      draw=red,
      thick,
      fill = white!80,
      rectangle,
      text=red,
      font=\bfseries\LARGE,  % Make text bold & larger
      inner sep=5pt          % Extra padding inside the box
    ]
    at (0.85, 0.7) {($x,y$)};
    
    % 3) Static sound souce
    \draw[red, above,ultra thick] (0.13, 0.3) circle (0.05);
    \node[
      draw=red,
      thick,
      rectangle,
      fill = white!80,
      text=red,
      font=\bfseries\LARGE,  % Make text bold & larger
      inner sep=5pt          % Extra padding inside the box
    ]
    at (0.28, 0.4) {Static Sound Source};
    \node[
      draw=red,
      thick,
      rectangle,
      fill = white!80,
      text=red,
      font=\bfseries\LARGE,  % Make text bold & larger
      inner sep=5pt          % Extra padding inside the box
    ]
    at (0.25, 0.2) {($x^*,y^*$)};

    
  \end{scope}
\end{tikzpicture}

==> figures/tik-images/rot-mic-image.tex <==
\begin{tikzpicture}%
  % Place the PNG image as a node
  \node[anchor=south west, inner sep=0] (image) at (0,0) {%
    \includegraphics[width=0.6\textwidth]{figures/robot/rotating-sensor-6in-arm1.jpg}%
  };
  
  \begin{scope}[
    x={(image.south east)},%
    y={(image.north west)}
  ]
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % 1) Microphone
    \node[
      draw=red,
      thick,
      rectangle,
      fill = white!80,
      text=red,
      font=\bfseries\LARGE,  % Make text bold & larger
      inner sep=5pt          % Extra padding inside the box
    ]
    at (0.35, 0.95) (mic-arm) {Microphone w/Rotating Arm};
    \draw[red, above,ultra thick] (0.33, 0.8) circle (0.03);
    \draw[->,red, ultra thick] (mic-arm.south) -- (0.33,0.83);


    %%%%%%%%%%%%%%%%%Y%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % 2) Servo motor
    \node[
      draw=red,
      thick,
      rectangle,
      fill = white!80,
      text=red,
      font=\bfseries\LARGE,  % Make text bold & larger
      inner sep=5pt          % Extra padding inside the box
    ]
    at (0.83, 0.88) (servo) {Servo Motor};
    \draw[red, above,ultra thick] (0.8, 0.68) circle (0.03);
    \draw[->,red, ultra thick] (servo.south) -- (0.8,0.71);
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % 3) DaqHat MCC172 label
    \node[
      draw=red,
      thick,
      rectangle,
      fill = white!80,
      text=red,
      font=\bfseries\LARGE,  % Make text bold & larger
      inner sep=5pt          % Extra padding inside the box
    ]
    at (0.23, 0.4) (daq172) {DaqHat MCC172};
    \draw[red, right,ultra thick] (0.9,0.4) circle (0.03);
    \draw[->,red,ultra thick] (daq172.east) -- (0.87,0.4);
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % 4) Raspberry pi 
    \node[
      draw=red,
      thick,
      rectangle,
      fill = white!80,
      text=red,
      font=\bfseries\LARGE,  % Make text bold & larger
      inner sep=5pt          % Extra padding inside the box
    ]
    at (0.2, 0.25) (rasppi) {RaspberryPi};
    \draw[red, right,ultra thick] (0.85,0.35) circle (0.03); 
    \draw[->,red,ultra thick] (rasppi.east) -- (0.82,0.35);
    
  \end{scope}
\end{tikzpicture}
